Noise Tolerant Identification and Tuning Approach Using Deep Neural Networks For Visual Servoing Applications

Vision based control of Unmanned Aerial Vehicles (UAVs) has been adopted by a wide range of applications due to the availability of low-cost on-board sensors and computers. Tuning such systems to work properly requires extensive domain specific experience, which limits the growth of emerging applications. Moreover, obtaining performance limits of UAV based visual servoing is difficult due to the complexity of the models used. In this paper, we propose a novel noise tolerant approach for real-time identification and tuning of visual servoing systems, based on deep neural networks (DNN) classification of system response generated by the modified relay feedback test (MRFT). The proposed method, called DNN with noise protected MRFT (DNN-NP-MRFT), can be used with a multitude of vision sensors and estimation algorithms despite the high levels of sensor's noise. Response of DNN-NP-MRFT to noise perturbations is investigated and its effect on identification and tuning performance is analyzed. The proposed DNN-NP-MRFT is able to detect performance changes due to the use of high latency vision sensors, or due to the integration of inertial measurement unit (IMU) measurements in the UAV states estimation. Experimental identification closely matches simulation results, which can be used to explain system behaviour and predict the closed loop performance limits for a given hardware and software setup. We also demonstrate the ability of DNN-NP-MRFT tuned UAVs to reject external disturbances like wind, or human push and pull. Finally, we discuss the advantages of the proposed DNN-NP-MRFT visual servoing design approach compared with other approaches in literature.

==> literature_summary.tex <==
Ground Target Tracking Control System for Unmanned Aerial Vehicles - Fixed wing. Assumes autopilot controller to accept velocity commands.
@article{oliveira2013ground,
  title={Ground target tracking control system for unmanned aerial vehicles},
  author={Oliveira, Tiago and Encarna{\c{c}}{\~a}o, Pedro},
  journal={Journal of Intelligent \& Robotic Systems},
  volume={69},
  number={1},
  pages={373--387},
  year={2013},
  publisher={Springer}
}

Fuzzy logic controller for predictive vision-based target tracking with an unmanned aerial vehicle. Quadrotor, poor performance, compared PD vs FLC vs FLC DES.
@article{harik2017fuzzy,
  title={Fuzzy logic controller for predictive vision-based target tracking with an unmanned aerial vehicle},
  author={Harik, El Houssein Chouaib and Guerin, Francois and Guinand, Fr{\'e}d{\'e}ric and Breth{\'e}, Jean-Fran{\c{c}}ois and Pelvillain, Herv{\'e} and Par{\'e}d{\'e}, Jean-Yves},
  journal={Advanced Robotics},
  volume={31},
  number={7},
  pages={368--381},
  year={2017},
  publisher={Taylor \& Francis}
}

Autonomous Landing of a Multirotor Micro Air Vehicle on a High Velocity Ground Vehicle. PID at close proximity with feedback linearization, DJI Matrice 100. Target velocity was up to 50km/h moving along a straight path. Manual tuning.
@article{borowczyk2017autonomous,
  title={Autonomous landing of a multirotor micro air vehicle on a high velocity ground vehicle},
  author={Borowczyk, Alexandre and Nguyen, Duc-Tien and Phu-Van Nguyen, Andr{\'e} and Nguyen, Dang Quang and Saussi{\'e}, David and Le Ny, Jerome},
  journal={Ifac-Papersonline},
  volume={50},
  number={1},
  pages={10488--10494},
  year={2017},
  publisher={Elsevier}
}


Visual Target Tracking and Relative Navigation for Unmanned Aerial Vehicles in a GPS-Denied Environment. Fixed Wing. Flight controller with its own PIDs.
@article{kim2014visual,
  title={Visual target tracking and relative navigation for unmanned aerial vehicles in a GPS-denied environment},
  author={Kim, Youngjoo and Jung, Wooyoung and Bang, Hyochoong},
  journal={International Journal of Aeronautical and Space Sciences},
  volume={15},
  number={3},
  pages={258--266},
  year={2014},
  publisher={The Korean Society for Aeronautical and Space Sciences}
}


Vision based autonomous landing of multirotor UAV on moving platform. PID controllers that are manually tuned, slowly moving target.
@article{araar2017vision,
  title={Vision based autonomous landing of multirotor UAV on moving platform},
  author={Araar, Oualid and Aouf, Nabil and Vitanov, Ivan},
  journal={Journal of Intelligent \& Robotic Systems},
  volume={85},
  number={2},
  pages={369--384},
  year={2017},
  publisher={Springer}
}


An Autonomous Vision-Based Target Tracking System for Rotorcraft Unmanned Aerial Vehicles. Nonlinear controller. Low speed tracking of a moving pedestrian:
One of critical concerns of the control system is the adjustment of the controller’s parameters. There are nine parameters in the PID algorithm, and it is quite difficult to adjust the parameters to achieve satisfactory control performance. In contrast, there are only two parameters to be adjusted in the proposed nonlinear controller, the two parameters can be set in a relatively wide range. The nonlinear controller is hence more conveniently implemented than the PID controller in real-world applications.

@inproceedings{cheng2017autonomous,
  title={An autonomous vision-based target tracking system for rotorcraft unmanned aerial vehicles},
  author={Cheng, Hui and Lin, Lishan and Zheng, Zhuoqi and Guan, Yuwei and Liu, Zhongchang},
  booktitle={2017 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={1732--1738},
  year={2017},
  organization={IEEE}
}


Vision-Based Target Tracking and Autonomous Landing of a Quadrotor on a Ground Vehicle. Linear controller augmented with a feedback linearization control law.
@inproceedings{hoang2017vision,
  title={Vision-based target tracking and autonomous landing of a quadrotor on a ground vehicle},
  author={Hoang, Tru and Bayasgalan, Enkhmurun and Wang, Ziyin and Tsechpenakis, Gavriil and Panagou, Dimitra},
  booktitle={2017 American Control Conference (ACC)},
  pages={5580--5585},
  year={2017},
  organization={IEEE}
}


Vision-Based Target Three-Dimensional Geolocation Using Unmanned Aerial Vehicles. Assumed controller of PixHawk. Loitering and hovering over target.
@article{zhang2018vision,
  title={Vision-based target three-dimensional geolocation using unmanned aerial vehicles},
  author={Zhang, Lele and Deng, Fang and Chen, Jie and Bi, Yingcai and Phang, Swee King and Chen, Xudong and Chen, Ben M},
  journal={IEEE Transactions on Industrial Electronics},
  volume={65},
  number={10},
  pages={8052--8061},
  year={2018},
  publisher={IEEE}
}
